Inspecting state of the art performance and NLP metrics in image-based medical report generation

Several deep learning architectures have been proposed over the last years to deal with the problem of generating a written report given an imaging exam as input. Most works evaluate the generated reports using standard Natural Language Processing (NLP) metrics (e.g. BLEU, ROUGE), reporting significant progress. In this article, we contrast this progress by comparing state of the art (SOTA) models against weak baselines. We show that simple and even naive approaches yield near SOTA performance on most traditional NLP metrics. We conclude that evaluation methods in this task should be further studied towards correctly measuring clinical accuracy, ideally involving physicians to contribute to this end.

==> LatinXAI abstract - v3/results-table.tex <==

\newcommand{\firstBest}[1]{\textbf{#1}}
\newcommand{\secondBest}[1]{\textbf{#1}}
\newcommand{\thirdBest}[1]{\textbf{#1}}

\begin{table}[!htbp]
\begin{center}
% \scriptsize

\caption{\centering Model performance in the IU X-ray dataset \cite{10.1093/jamia/ocv080}.
Results are taken from each paper, except for TieNet which are taken from Liu et al. \cite{liu2019clinically}.
% Notice each author used their own test split.
B: BLEU, R-L: ROUGE-L, C-D: CIDEr-D.
% Accuracy and AUC are calculated with the Chexpert labeler.
}
%\vspace{-5mm}
\begin{tabular}{lccccccccc}
\toprule
Model &  B-1 &  B-2 &  B-3 &  B-4 &  B &  R-L &  C-D &   Acc &  AUC \\
\midrule
Liu et al. \cite{liu2019clinically}  &  0.369 &  0.246 &  0.171 &  0.115 & 0.225 &   \secondBest{0.359} &   \firstBest{1.490} & \secondBest{0.916} &    - \\
TieNet \cite{wang2018tienet} & 0.330 & 0.194 & 0.124 & 0.081 & 0.182 & 0.311 & \secondBest{1.335} & 0.902 & - \\
KERP \cite{li2019knowledge} & \firstBest{0.482} & \secondBest{0.325} & \secondBest{0.226} & \thirdBest{0.162} & \secondBest{0.298} & 0.339 & 0.280 & - & - \\
Xue et al. \cite{xue2019features} & \secondBest{0.477} & \firstBest{0.332} & \firstBest{0.243} & \firstBest{0.189} & \firstBest{0.310} & \firstBest{0.380} & - & - & - \\
\hline % midrule
Constant  &  \thirdBest{0.455} &  \thirdBest{0.312} &  \thirdBest{0.223} &  \secondBest{0.165} & \thirdBest{0.289} &   \thirdBest{0.357} &   \thirdBest{0.293} & \thirdBest{0.915} &    0.500 \\
Random    &  0.362 &  0.197 &  0.117 &  0.075 & 0.188 &   0.264 &   0.112 & 0.894 &    0.508 \\
Nearest-neighbor       &  0.383 &  0.220 &  0.142 &  0.100 & 0.211 &   0.288 &   0.230 & 0.903 &    \firstBest{0.518} \\
% top-s-10  &  0.275 &  0.170 &  0.113 &  0.078 & 0.159 &   0.294 &   0.152 & 0.915 &    0.500 \\
% top-s-50  &  0.333 &  0.206 &  0.137 &  0.097 & 0.193 &   0.283 &   0.188 & 0.911 &    0.500 \\
Top-sentences-100 &  0.347 &  0.211 &  0.138 &  0.096 & 0.198 &   0.281 &   0.166 & 0.911 &    0.498 \\ % top-s-100
% top-w-10  &  0.312 &  0.108 &  0.024 &  0.000 & 0.111 &   0.244 &   0.043 & 0.915 &    0.500 \\
Top-words-50  &  0.375 &  0.102 &  0.019 &  0.000 & 0.124 &   0.224 &   0.075 & 0.835 &    \secondBest{0.509} \\ % top-w-50
% top-w-100 &  0.349 &  0.090 &  0.016 &  0.000 & 0.114 &   0.206 &   0.072 & 0.820 &    0.483 \\
\hline % midrule
CNN-LSTM      &  0.379 &  0.239 &  0.164 &  0.117 & 0.225 &   0.338 &   0.284 & 0.912 &    0.505 \\
CNN-LSTM-att  &  0.361 &  0.226 &  0.152 &  0.106 & 0.211 &   0.314 &   0.187 & \firstBest{0.918} &    \thirdBest{0.508} \\
\bottomrule
\end{tabular}

    \label{table:results}
    \end{center}
\end{table}
